High-quality Surface Reconstruction using Gaussian Surfels

We propose a novel point-based representation, Gaussian surfels, to combine the advantages of the flexible optimization procedure in 3D Gaussian points and the surface alignment property of surfels. This is achieved by directly setting the z-scale of 3D Gaussian points to 0, effectively flattening the original 3D ellipsoid into a 2D ellipse. Such a design provides clear guidance to the optimizer. By treating the local z-axis as the normal direction, it greatly improves optimization stability and surface alignment. While the derivatives to the local z-axis computed from the covariance matrix are zero in this setting, we design a self-supervised normal-depth consistency loss to remedy this issue. Monocular normal priors and foreground masks are incorporated to enhance the quality of the reconstruction, mitigating issues related to highlights and background. We propose a volumetric cutting method to aggregate the information of Gaussian surfels so as to remove erroneous points in depth maps generated by alpha blending. Finally, we apply screened Poisson reconstruction method to the fused depth maps to extract the surface mesh. Experimental results show that our method demonstrates superior performance in surface reconstruction compared to state-of-the-art neural volume rendering and point-based rendering methods.

==> src/tex/backup.tex <==
\section{Related Work}

Multi-view surface reconstruction methods use two-dimensional images of an object or scene to create its geometric representation. Traditional approaches employ multi-view stereo (MVS) techniques \cite{}, such as voxel grids optimization \cite{}, feature point growing \cite{}, or depth-map estimation and merging \cite{}. These methods depend on photometric consistency across views, which may pose challenges in accurately capturing intricate geometric details. 

Recently, differentiable rendering \cite{} has shown powerful capabilities in view synthesis and surface reconstruction. By directly minimizing the per-pixel difference between the image and rendering results, it can reconstruct surfaces with fine details \cite{} and adapt to complex materials through a sophisticated rendering process \cite{}.

% I think volumetric rendering is a key different
\subsection{Neural volume rendering}

% In recent years, differentiable rendering \cite{} has demonstrated powerful capabilities in view synthesis and surface reconstruction. By directly minimizing the per-pixel difference between the image and rendering results, it can reconstruct surfaces with fine details and complex materials through a sophisticated rendering process \cite{}.

Based on scene representation, current differentiable rendering can be broadly categorized into two types: neural volume rendering and neural point-based rendering.

The landmark work in neural volume rendering is NeRF~\cite{}, which employed a differentiable volumetric rendering technique to reconstruct a neural scene representation, achieving impressive photorealistic view synthesis with view-dependent effects. To accelerate its optimization, subsequent research replaces the neural scene representation with explicit or hybrid scene representations, such as voxel grids~\cite{karnewar2022relu, sun2021direct, yu2021plenoxels}, low-rank tensors~\cite{chen2022tensorf}, tri-planescite{chan2022efficient, reiser2023merf, zhang2023efficient}, and multi-resolution hash mapscite{mueller2022instant}. 

However, NeRF and its variants extract isosurfaces based on heuristic thresholding of density values, introducing high-frequency noise in the reconstructed surfaces. To enhance reconstruction quality, some studies suggest using occupancy grids \cite{} or signed distance functions (SDFs) \cite{} which can provide better-defined 3D surfaces compared to volume density fields.

% These approaches have led to significant improvements in the training speed of neural representations.
% The scene representation employs an MLP network to map 3D spatial locations to color and volume density. Later, the explicit scene representation or hybrid scene representation.
% A problem of NeRF and its variants [1,30,43,46],
% however, is the question of how an isosurface of the volume density could be defined to represent the underlying 3D geometry. Current practice often relies on heuristic thresholding on the density values; due to insufficient constraints
% on the level sets, however, such surfaces are often noisy and may not model the scene structures accurately.

% To integrate with neural volume rendering [22], different techniques [36, 41] have been proposed to reparametrize the underlying representations back to volume density. These designs of neural implicit functions enable more accurate surface prediction with view synthesis capabilities of unsacrificed quality [42]

Follow-up works enhance reconstruction by utilizing auxiliary information \cite{}. NeuralWarp \cite{} employs patch warping with co-visibility information for surface optimization. Monocular depth and normals \cite{}, sparse point clouds \cite{Geo-neus, RegSDF}, semantic segmentation \cite{}, and geometric priors \cite{} are also employed to guide and regularize 3D reconstruction.

% Follow-up works extend the aforementioned approaches by utilizing auxiliary information to enhance the reconstruction results \cite{}. NeuralWarp \cite{} employs patch warping with co-visibility information to guide surface optimization. Additionally, the use of monocular depth and normals \cite{}, parse point clouds \cite{Geo-neus,RegSDF}, semantic segmentation \cite{}, geometric priors \cite{} as auxiliary data has been explored to regularize 3D reconstruction, enhancing the robustness of surface reconstruction. 

On the other hand, some methods incorporate explicit voxel grids \cite{Voxurf} or multi-resolution hash encodings with CUDA-based MLPs to expedite surface reconstruction \cite{}. For calculating the derivatives of Eikonal loss, Instant-NSR \cite{} approximates these derivatives using finite differences, while NeuS2 \cite{} proposes a precise and efficient formulation of second-order derivatives tailored to MLPs. Neuralangelo \cite{} also utilizes numerical gradients for computing higher-order derivatives as a smoothing operation. Additionally, it involves coarse-to-fine optimization on the hash grids, controlling different levels of details.

% Neuralangelo [27] presents a novel method that leverages multi-resolution hash grids with numerical gradient computation for neural surface reconstruction. Similar are adopted by Instant-NSR and NeuS2

% the key challenge of adding the
% Eikonal loss to CUDA-based MLPs (a key factor to fast
% training in Instant-NGP [37]) is how to calculate the secondorder derivatives efficiently for backpropagation. InstantNSR [71] addresses this by approximating the second-order
% derivatives using finite differences, which suffer from precision problems and it can cause unstable training. Instead,
% we propose a simple, precise,

% NeuS2

% Instant-NSR

% is how to calculate the secondorder derivatives efficiently for backpropagation. Instant-NSR [71] addresses this by approximating the second-order derivatives using finite differences, which suffer from precision problems and it can cause unstable training. Instead,
% we propose a simple, precise, and efficient formulation of
% second-order derivatives tailored to MLPs (Sec. 4.2), which
% leads to fast and high-quality reconstruction. 

% some works propse to incorporating explicit voxel grids \cite{} or multi-resolutio hash encodings \cite{}.

%  leverages multi-resolution hash grids

% Other works extend the aforementioned approaches to accelerate optimization by incorporating explicit voxel grids \cite{} or hash encodings \cite{}.

% Voxurf [61] proposes a voxel-based
% surface representation for fast multi-view 3D reconstruction. While it enables 20x speedup over the baseline (i.e.,
% NeuS [59]), our proposed method is over 3x faster than Voxurf and achieves better geometry quality when compared
% with Voxurf’s results reported in their paper, as shown in
% the Suppl. document. Neuralangelo [27] presents a novel

% Follow-up works extend the aforementioned approaches by utilizing auxiliary information to enhance the reconstruction results \cite{}. NeuralWarp \cite{} employs patch warping with co-visibility information to guide surface optimization. Geo-neus \cite{} and \cite{} RegSDF leverage sparse point clouds from SfM to supervise the SDF. Additionally, the use of monocular depth and normals \cite{}, semantic segmentation \cite{}, geometric priors \cite{} as auxiliary data has been explored to regularize 3D reconstruction, enhancing the robustness of surface reconstruction. Other works extend the aforementioned approaches to accelerate optimization by incorporating explicit voxel grids \cite{} or hash encodings \cite{}.

\subsection{Neural point-based rendering.}

 While true to the
underlying data, point sample rendering suffers from holes, causes
aliasing, and is strictly discontinuous. Seminal work on high-quality
point-based rendering addresses these issues by “splatting” point
primitives with an extent larger than a pixel, e.g., circular or elliptic
discs, ellipsoids, or surfels [Botsch et al. 2005; Pfister et al. 2000; Ren
et al. 2002; Zwicker et al. 2001b].

Yifan et al. [44] propose a
point-based representation with a position and normal parameterization. Each point is rendered as a small ‘surface’
with position, radius, and normal. In the examples shown in
their paper, they use representations with up to 100k points
and report orders of magnitude slower runtime than our approach (258 ms forward and 680 ms backward for an image
of resolution 256 × 256 pixels). Lin et al. [13] define a
renderer for point cloud generation, but only provide gradients for depth values. Roveri et al. [29] define a pointbased differentiable projection module for neural networks
that produces ‘soft’ depth images. Aliev et al. [2] propose to
model room-scale point clouds with a deferred neural rendering step. SynSin [42] and the PyTorch3D point renderer
follow a similar approach to ours, but are orders of magnitude slower. In addition, we employ a different blending
function and enable the optimization of the sphere radius.
Furthermore, they use only the first few points per pixel to
determine the pixel colors. We have found this to leads to
high frequency artifacts in complex scenes and thus allow
for an unlimited number of spheres to contribute to the pixel
color (or set a bound based on the minimum contribution)
and use only the first few spheres for gradient propagation.


% Recently, NeRF adopts differentiable volumetric rendering technique to reconstruct a nerual-based volumatric scene representation, achieves remarkable photorealistic view synthesis with view-dependent
% effects.. The representation encodes 3D scenes with an MLP mapping 3D spatial locations to color and volume density

% NeRF achieves remarkable photorealistic view synthesis with view-dependent
% effects. NeRF encodes 3D scenes with an MLP mapping 3D
% spatial locations to color and volume density. These predictions are composited into pixel colors using neural volume
% rendering. A problem of NeRF and its variants [1,30,43,46],
% however, is the question of how an isosurface of the volume density could be defined to represent the underlying 3D
% geometry. Current practice often relies on heuristic thresholding on the density values; due to insufficient constraints
% on the level sets, however, such surfaces are often noisy
% and may not model the scene structures accurately [36, 41].
% Therefore, more direct modeling of surfaces is preferred for
% photogrammetric surface reconstruction problems.


% Volumetric methods use voxel
% grids, multiplane images, or neural networks to represent
% scenes as continuous volumetric functions of density and
% color. Recently, Neural Radiance Fields (NeRF) [22] introduced a novel scene representation based on a continuous
% volumetric function parameterized by a multilayer perceptron (MLP). NeRF produces photorealistic renderings with
% fine details and view-dependent effects, achieved through
% volumetric ray tracing. However, the original NeRF is computationally expensive and memory intensive









% Multi-view surface reconstruction methods rely on a set of two-dimensional images of a object or scene to generate a geometric representation
% of the object or scene. Traditional methods employ multi-view stereo (MVS) methods produced impressive full 3D reconstruction algorithms over the years via voxel grids, surface evolution based
% methods, feature point growing, and depth-map estimation and merging.


% All these methods re-project and
% blend the input images into the novel view camera, and use the
% geometry to guide this re-projection. These methods produced excellent results in many cases, but typically cannot completely recover from unreconstructed regions, or from “over-reconstruction”,
% when MVS generates inexistent geometry. Recent neural rendering algorithms [Tewari et al. 2022] vastly reduce such artifacts and
% avoid the overwhelming cost of storing all input images on the GPU,
% outperforming these methods on most fronts.

% Early image-based photogrammetry techniques use a volumetric occupancy grid to

% use voxel grids, multiplane images, 

% represent the scene [4, 16, 17, 29, 32]. Each voxel is visited
% and marked occupied if strict color constancy between the
% corresponding projected image pixels is satisfied. The photometric consistency assumption typically fails due to autoexposure or non-Lambertian materials, which are ubiquitous
% in the real world. Relaxing such color constancy constraints
% across views is important for realistic 3D reconstruction.


% The very first novelview synthesis approaches were based on light fields [19],
% and developed the concept of volume rendering for novel
% views. Their work emphasized the importance of efficiently
% traversing volumetric data to produce realistic images.
% Various scene representations have been proposed since,
% such as triangle meshes, point clouds, voxel grids, multiplane images, or neural implicit functions.

% Early image-based photogrammetry techniques use a volumetric occupancy grid to
% represent the scene [4, 16, 17, 29, 32]. Each voxel is visited
% and marked occupied if strict color constancy between the
% corresponding projected image pixels is satisfied. The photometric consistency assumption typically fails due to autoexposure or non-Lambertian materials, which are ubiquitous
% in the real world. Relaxing such color constancy constraints
% across views is important for realistic 3D reconstruction.

% Image-based rendering (IBR) methods rely on a set of two-dimensional images of a scene to generate a representation
% of the scene and render novel views. The very first novelview synthesis approaches were based on light fields [19],
% and developed the concept of volume rendering for novel
% views. Their work emphasized the importance of efficiently
% traversing volumetric data to produce realistic images.
% Various scene representations have been proposed since,
% such as triangle meshes, point clouds, voxel grids, multiplane images, or neural implicit function



% Volumetric methods use voxel grids, multiplane images, 


% or neural networks to represent
% scenes as continuous volumetric functions of density and
% color. Recently, Neural Radiance Fields (NeRF) [22] introduced a novel scene representation based on a continuous
% volumetric function parameterized by a multilayer perceptron (MLP). NeRF produces photorealistic renderings with
% fine details and view-dependent effects, achieved through
% volumetric ray tracing. However, the original NeRF is computationally expensive and memory intensive.

% Early image-based photogrammetry techniques use a volumetric occupancy grid to represent the scene. Each voxel is visited and marked occupied if strict color constancy between the
% corresponding projected image pixels is satisfied. The photometric consistency assumption typically fails due to auto-exposure or non-Lambertian materials, which are ubiquitous
% in the real world. Relaxing such color constancy constraints
% across views is important for realistic 3D reconstruction.

% \subsection{Point-based surface reconstruction.}

% The 3DGS [25], as a special point-based rendering, stands out for its distinctive utilization of explicit representation and differential
% point-based splatting techniques, thereby facilitating realtime rendering at novel views. However, it’s difficult to
% directly regress 3D Gaussians from image for high-quality
% novel view synthesis. In this paper, we leverage a hybrid
% 3D representation, facilitating fast and generalizable reconstruction and rendering




% Point-based IBR methods. Alternatively, point-based
% representations for radiance field excel at modeling thin geometry and leverage fast point rasterization pipelines to render images using α-blending rather than ray-marching [17,
% 31]. In particular, the very recent 3D Gaussian Splatting
% model [15] allows for optimizing and rendering scenes with
% speed and quality never seen before.


% represent the center position and the rotation represented by a quaternion. $\mathbf{s}_p \in \mathbb{R}^3$ represent the scaling factors for each axis. $\mathbf{\Sigma}_p \in \mathbb{R}$ and $\mathcal{C}_p \in \mathbb{R}^k$ represent opacities and spherical harmonic coefficients of each Gaussian. The difference between our 2D Gaussian kernels with 3DGS \cite{} is that our scaling faceors $\mathbf{s}_p=[\mathbf{s}^x_p,\mathbf{s}^y_p,0]$.


% $\sigma_p$,


% $\mathbf{\Sigma }_p$ and $\mathcal{C}_p$ represent the centers, rotation, scaling factors, 

% represented by a quaternion r ∈ R
% 4
% .


% opacities, covariance matrices, and spherical harmonic coefficients of the Gaussians. 

% The Gaussian kernels are transformed to camera space through a viewing transformation denoted by $\mathbf{W}$, and subsequently to image space using the Jacobian of the affine approximation of the projective transformation, denoted as $\mathbf{J}$. The transformed covariance
% matrix $\mathbf{\Sigma}'$ in camera coordinates 
% can be determined as:
% \begin{align}
% G'\left( \mathbf{u};\mathbf{u}_p,\mathbf{\Sigma }'_p \right) &=\exp \left\{ -\small{\frac{1}{2}\left( \mathbf{u}-\mathbf{u}_p \right) ^{\top}}{\mathbf{\Sigma}'_p}^{-1}\left( \mathbf{u}-\mathbf{u}_p \right) \right\} \\
% \mathbf{\Sigma }'_p&=\left( \mathbf{J}_k\mathbf{W}_k\mathbf{\Sigma }_p\mathbf{W}_{k}^{\top}\mathbf{J}_{k}^{\top} \right) \left[:2,:2\right]
% \end{align}
% The 2D Gaussian kernels are defined in 3D space, represented as:
% \begin{align}
% G\left( \mathbf{x} \right) =\exp \left\{ -\small{\frac{1}{2}\left( \mathbf{x}-\mathbf{x}_p \right) ^{\top}}{\mathbf{\Sigma }_p}^{-1}\left( \mathbf{x}-\mathbf{x}_p \right) \right\}
% \end{align}
% \paragraph{Differentiable Rendering}
% Regularization for 3D Gaussians
% \subsection{Optimization}
% \paragraph{Rendering}

% \jiamin{If the normal is correct but depth is not, it can be seen as normal-aware depth smoothing. It the depth is correct and normal are not, .... Note that according to the chain role, the gradient with respect to normal the 3rd colome of R is zero.}
% As we observe in experiments that the point normal is tend to be noisy and sometimes deteriorates the optimization, we further adopt a curvature smooth loss by slightly punishing the image-space gradients of the rendered normal $\nabla{\tilde{N}}$:
% \begin{align} \label{eq:loss_geom}
% \mathcal{L}_{\mathrm{c}}=\lambda_{g}L_1(\tilde{N}, \nabla{\tilde{D}})+{\lambda_{c}}L_1(\nabla{\tilde{N}}, \mathbf{0}).
% \end{align}
% As we observe in experiments that the point normal is tend to be noisy and sometimes deteriorates the optimization, we further adopt a curvature smooth loss by slightly punishing the image-space gradients of the rendered normal $\nabla{\tilde{N}}$:
% Gaussian points are very fast to optimize as they explicitly represent the scene radiance using SH-coded features. However, such explicitation and the low representation ability of SH make the model prune to highly view-dependent signals that vary drastically with respect to changing viewing directions. As a consequence, the model would resort to explaining highlights or reflections using the point geometry and then causes holes and floaters in the reconstructed mesh[fig: no prior holes]. To this end, we integrate a pretrained normal predictor to guide the point normal optimization:
% \begin{align} \label{eq:loss_prior}
% \mathcal{L}_{\mathrm{n}}=\lambda_{p}L_1(\tilde{N}, \hat{N}),
% \end{align}
% where $\hat{N}$ is the normal predicted by the prior model[cite: omnidata]. We found such a normal prior loss largely helps to recover the true geometry for scenes with strong highlights where the rendering loss fails to find photo-consistency between images.

% per-pix depth
% prior is not always activated

\section{Introduction}

Multi-view surface reconstruction stands as a foundational task in the realm of 3D computer vision. 

% The conventional pipeline typically involves the structure from motion (SfM) procedure, which jointly provides calibrated camera poses for the images and a sparse point cloud. Additionally, multi-view stereo (MVS) techniques are employed to generate a dense point cloud through dense image-space feature matching. In recent years, competitive alternatives, such as neural radiance fields (NeRF) \cite{} and differentiable rendering, have emerged in the domain of view synthesis and 3D reconstruction. These approaches utilize either voxel-based implicit representation \cite{} or neural implicit representation \cite{}, proving particularly effective in scenarios featuring texture-less surfaces and complex materials.

Following NeRF and its variations \cite{}, 3D Gaussian Splatting (3DGS) \cite{} has gained widespread popularity for capturing and rendering 3D scenes. Different from mesh-based representations \cite{} and voxel-based or neural-based implicit representations \cite{}, 3DGS captures the appearance and geometry through a set of topology-free Gaussian points. This approach can adding and occasional removing 3D Gaussian points adaptively during optimization, which offers greater flexibility to significantly improve the quality of recon than mesh-based methods, which. Additionally, as an explicit representation, 3DGS utilizes explicit Gaussian kernels to prevent point sampling, proving more efficiency in both training and rendering when compared with voxel-based or neural-based implicit representations. xxx in xxx mininus and real-time rendering

% The advantage of the 3D Gaussian Splatting [18] is that
% it can generate dense point clouds with detailed geometry,
% which provides sufficient geometric constraints especially
% for regions with intricate details. However,

Despite the advantages of the 3DGS representation, the basic 3D Gaussian Splatting, even with realistic rendering results, struggles to directly generate high-quality reconstructions. As shown in Fig. \ref{fig:teaser}, the 3D Gaussians, resembling 3D ellipsoids, are not closely aligned with the actual surfaces. This limitation stems from two aspects: 1. Fitting ellipsoids to a surface in a 2D manifold proves challenging, \jiamin{ normal can not accurate opt} 2. The rendering of 3DGS relies on alpha-blending, introducing shape-radiance ambiguities \cite{zhang2020nerf++} similar to NeRF. This may lead to the emergence of ``foggy'' geometry. \cite{} and \cite{}, xxx remains challenging.

To mitigate this problem, we propose a flattened Gaussian representation defined on a 2D elliptical disk instead of a 3D ellipsoid, ensuring that the points are in close proximity to the surface. Moreover this enhancement can also contributes to better color consistency in novel view rendering.

Contrasted with 3D Gaussian-based radiance field rendering, employing flattened Gaussians for precise surface representation with fine details requires more accurate position, scaling, and normal for each Gaussian kernel. To achieve this, we regularize the normal direction by aligning it with the monocular estimated normal and ensuring consistency with the rendered depth map. Another challenge for flattened Gaussians is representing sharp depth discontinuities. If the flattened Gaussians extend beyond the actual boundary, their weight can impact the rendered depth, potentially degrading the quality of the reconstruction. To address this, we propose a cutoff schedule that prunes incorrect points near depth edges. An illustration of our proposed flattened Gaussian reconstruction is shown in Fig. \ref{fig:teaser}.


In summary, our contributions include:
\begin{itemize}[leftmargin=12pt,topsep=4pt]
\item We present a novel approach utilizing a flattened 3D Gaussian representation designed to closely adhere to the actual surface. This technique can enhance both the efficiency and precision of surface reconstruction while achieving better consistency in view synthesis.

\item We introduce a depth-normal consistent regularizer to address the ambiguity between the depth and normal of the flattened 3D Gaussian. This is crucial for achieving accurate position and orientation for the Gaussians. \jiamin{shall we  define a depth-normal ambiguity?}

\item The Chamfer distance of the reconstruction increases by xx\% to xx\%, and the PSNR of rendered images improves by xx\% to xx\% on the xxx and xxx datasets,  with high-frequency geometric details (Fig. \ref{fig:teaser}).
\end{itemize}

% As we employ pixel-wise photometric loss and enforce depth-normal consistency during optimization, we have observed that the rendered depth image can capture more details than the direct mesh extraction from the Gaussian point cloud results. Therefore, we first render depth and normal maps to each input view, back-project the each depth and normal map to point clouds with normal, and fuse the point cloud of all views using Screened Poisson Reconstruction \citeP{} to extract meshing.


% and fuse the per-pixel points into a global point cloud, and then apply Screened Poisson meshing[cite:screened poisson] on the fused points.
% The fused point cloud more fits the learned geometry surface better and is also more evenly-distributed. 
% However, for 3D regions with abrupt depth change like sharp edges, the continuously changing value in depth maps results in outlier points especially in scenes with complex occlusions[fig: edge depth ambig]. Thus, we adopt a point pruning process before meshing.

% Direct reconstruction from Gaussian point cloud results in pool quality mesh[fig: direct poisson], as it treats each Gaussian as a simple point without considering the properties of scales, rotation, and opacity. Therefore, we first render depth and normal maps from given views and fuse the per-pixel directional points into a global point cloud, and then apply Screened Poisson meshing[cite:screened poisson] on the fused points.
% The fused point cloud more fits the learned geometry surface better and is also more evenly-distributed. 
% However, for 3D regions with abrupt depth change like sharp edges, the continuously changing value in depth maps results in outlier points especially in scenes with complex occlusions[fig: edge depth ambig]. Thus, we adopt a point pruning process before meshing.
% \begin{figure}[h]
%   \centering
%   \includegraphics[width=.98\linewidth]{}
%   \caption {\label{fig:}
%   edge ambiguity}
% \end{figure}
% We have omitted one dimension of scaling from 3D Gaussian kernel to reduce depth ambiguity, but there is still ambiguity in depth around sharp edges. 



% Specifically, we first construct a $512 \times 512 \times 512$ voxel grids within the bounding box of 3D point cloud. For each flattened Gaussians, we calculated its intersected voxel grids and calculate its $\alpha_{i}$, which is calculated between the center point of each voxel grid and the Gaussian. Then for each voxel, we sum up the $\alpha_{i}$ of all the intersected Gaussian kernels and prune the voxels whose aggregated alpha values lower than $\lambda=1$, set the remaining voxels as valid voxels. Then for each view, we remove point cloud that is not within valid voxels.

% This is done by intersecting all flattened Gaussians as anisotropic "disks" in world space with a global volume to get an occupancy grid, where each voxel stores the sum of $\alpha_{i}$ of all intersected Gaussians. Then we use this occupancy grid to prune the fused points that locate in voxels with the aggregated occupancy values lower than $\lambda_{prune}=1$.

% The weight of each Gaussian kernel decays smoothly to almost zero with the sampling position moving away from the kernel center until the distance reaches a cutoff threshold. The smooth gradient of the Gaussian kernel is stable for optimization, but it is not capable of modeling abrupt depth change of geometry edges. Conversely, a lower cutoff distance has potential to represent sharp geometry, but we found it unstable to train in our experiments. 
% Therefore, we apply an additional cutoff on the learned Gaussians as a post process to prune the fused points.
% This is done by intersecting all flattened Gaussians as anisotropic "disks" in world space with a global volume to get an occupancy grid, where each voxel stores the sum of $\alpha_{i}$ of all intersected Gaussians. Then we use this occupancy grid to prune the fused points that locate in voxels with the aggregated occupancy values lower than $\lambda_{prune}=1$.

% used to project the image space coordinate $\mathbf{u}-\mathbf{u}_i$ to the tangent space and compensate for the depth offset to $d_i\left( \mathbf{u}_i \right)$ to obtain the true depth of intersection point.
% where $\mathbf{u}_0$ and $\mathbf{u}_1$ are unit basis vectors in screen space, and $\mathbf{R}_i^k$ denotes the $k_{th}$ column of $\mathbf{R}_i$. $\mathbf{R}_i^0$ and $\mathbf{R}_i^1$ together form a pair of coordinate bases on the local tangent plane. Once we have the differences of a pixel to the projected Gaussian center $\Delta\mathbf{u}$ in rendering path, we can efficiently compute per-pixel depth by adding a correction term to the depth of the Gaussian center $d_i$:

% Note that 
% When rendering a 3D Gaussian point, viewing rays traverse through the Gaussian kernel for a distance and there is no exact intersection between them (fig.~\ref{fig: 3d_depth_ambig}). While the intersection of a ray with the local tangent plane determined by our 2D Gaussian point can be computed exactly. 
% To this end, we first compute the local coordinates mapping of inverse projection $\mathbf{J}'$ from screen space to point tangent space[cite:surface-splatting] by:
% % \begin{align} \label{eq:inverse_prj}
% % \mathbf{J}'=\left ( \begin{matrix}
% %             \mathbf{u}_0{\cdot}\mathbf{R}_i[:,0], & \mathbf{u}_1{\cdot}\mathbf{R}_i[:,0] \\
% %             \mathbf{u}_0{\cdot}\mathbf{R}_i[:,1], & \mathbf{u}_1{\cdot}\mathbf{R}_i[:,1] \\
% % \end{matrix} \right ),
% % \end{align}
% where $\mathbf{u}_0$ and $\mathbf{u}_1$ are unit basis vectors in screen space, and $\mathbf{R}_i^k$ denotes the $k_{th}$ column of $\mathbf{R}_i$. $\mathbf{R}_i^0$ and $\mathbf{R}_i^1$ together form a pair of coordinate bases on the local tangent plane. Once we have the differences of a pixel to the projected Gaussian center $\Delta\mathbf{u}$ in rendering path, we can efficiently compute per-pixel depth by adding a correction term to the depth of the Gaussian center $d_i$:
% \begin{align} \label{eq:pix_depth}
% d_i\left( \mathbf{u} \right) =d_i\left( \mathbf{u}_i \right) +\mathbf{R}_i[2,:1]\mathbf{R}_{i}^{\top}\left[ :2,:2 \right] \left( \mathbf{u}-\mathbf{u}_i \right).
%     % d^{pix}_i=d_i+(\mathbf{R}_i[2,0],\mathbf{R}_i[2,1]){\cdot}\mathbf{J}'{\cdot}\Delta\mathbf{u}.
% \end{align}

% Based on the \textit{local homography} assumption[cite: surface-splatting], we compute the coordinate mapping Jacobian $\mathbf{J}$ from the point tangent plane to the image plane using local parameterization. This allows us to render more accurate per-pixel depth by forward differencing instead of approximating with the depth of Gaussian centers. This enables finer optimization and surpervision on the Gaussian depth. 

As shown in Fig. \ref{}, compared with calculating the median depth of all intersected Gaussian points, and considered the rendered depth whose far from (larger than $\lambda$) from the median depth as ourliders, our volumatric cutting process exhibits better quality and computational efficiency.


traversing the pixels in all depth images, calculating each weighted opacity $\alpha_{i}$ along the ray, and performing depth cutting, our voxel-based cutting process exhibits better computational efficiency, with $\mathrm{O}(n)$ complexity, where $n$ is the number of Gaussian points.

, with $\mathrm{O}(n)$ complexity, where $n$ is the number of Gaussian points

As a result, we utilize a volumetric cutting to remove false depth point. Spcifically, we utilize a voxel grid in 3D space to expedite the cutoff process. Specifically, we first construct a $512 \times 512 \times 512$ voxel grid within the bounding box. Next, we traverse all the Gaussian ellipse disks, calculate their intersection with the surrounding voxels, and accumulate the weighted opacity $\alpha_{i}$ to the corresponding voxels. To reduce computational cost, we approximate the integration of Gaussian weights and opacities within the intersection area using the $\alpha_{i}$ of the voxel center. Here, if a voxel has a low accumulate weighted opacity, lower than $\lambda=1$ in our experiments, it is near the foreground boundary (depth discontinuity) or far from the background surface, we will prune the points in these voxels. 

% We compare geometry reconstruction quality with two point-based methods: \textit{3D Gaussian}[cite:3dgs], \textit{SuGaR}[citd:sugar], \textit{Pulsar}[cite: pulsar], and three implicit SDF methods: \textit{NeuS}[cite:neus], \textit{Instant Neural Surface Reconstruction[cite:insr]}, \textit{Neuralangelo[cite:nrgl]}.

% We
% either extract the mesh using a very fine marching cubes
% algorithm [21], by applying Poisson reconstruction [14] using the centers of the 3D Gaussians as the surface point
% cloud, or by applying our mesh extraction method on different level sets. Quantitative results are available in Table 2
% and show the clear superiority of our approach for meshing
% 3D Gaussians. Figure 3 also illustrates how the marching
% cubes algorithm fails in this context

% our method can fast convergent to high-quality reconstruction. NueS leverages the inherent continuity of deep MLPs which is robost to outliers, but can resulting in smooth and complete surface representations. Our reconstruction speed is comparable with INSR and NeuS, which use hash feature maps and tiny MLPs to accerlarate the the implicit surface optimization. However, using our flattened Gaussian represention, our reconstruction quality are better than INSR and NeuS.

% which is comparable with NeuS2 
% Our rendered reflections are temporally smooth, unlike SVS. 
% For outdoor scenes, our method produces sharper details in the trees and background buildings (Fig. \ref{}b). 
% Our Block-NeRF implementation tends to produce blurry rendering results for distant objects because Block-NeRF does not have contraction mapping and samples distant objects with low density. 
% Similarly, Mega-NeRF also blurs distant objects despite using an unbound scene parameterization similar to NeRF++~\cite{zhang2020nerf++}. This is likely due to the use of a set of MLPs to represent the scene without a local feature grid, which can lead to slower optimization convergence.

% We compare our method to other state-of-the-art surface reconstruction methods both quantitatively and qualitatively. All comparisons use original author's implementations and hyperparameters.

% We follow previous works \cite{yariv2020multiview,wang2021neus} to use a subset with 15 different scenes for evaluation. The Chamfer distance is calculated between the masked ground truth point cloud and the vertices of the reconstructed mesh.

% As the DTU ground truth point cloud is incomplete in some region, we follow [cite: neuralWarp, neuralangelo] using a threshold to discard point pairs with distances larger than $cd_{max}$, here we choose $cd_{max}=10mm$. Note that Chamfer distance is often prone to outliers, please refer to qualitative results[ref:visual cmp] for visualized comparisons.
